A Grammatical Approach for Distributed Business Process Management using Structured and Cooperatively Edited Mobile Artifacts

In this thesis, we focus on the proposal of distributed workflow systems dedicated to the automation of administrative business processes. We propose an approach to build such systems by relying on the concepts of multiagent systems, Peer to Peer (P2P) architecture, Service-Oriented Architecture (SOA) and structured documents (artifacts) cooperative edition. Indeed, we develop mathematical tools that allow any workflow systems designer, to express each administrative process in the form of an attributed grammar whose symbols represent tasks to be executed, productions specify a scheduling of these tasks, and instances (the derivation trees that conform to it) represent the different execution scenarios leading to business goal states. The obtained grammatical model is then introduced into a proposed P2P system which is in charge of carrying out the completely decentralised execution of the underlying process's instances. The said system orchestrates a process's instance execution as a choreography during which, various software agents driven by human agents (actors), coordinate themselves through artifacts that they collectively edit. The exchanged artifacts represent the system's memory: they provide information on already executed tasks, on those ready to be executed and on their executors. The software agents are autonomous and identical: they execute the same unique protocol each time they receive an artifact. This protocol allows them to identify the tasks they must immediately execute, to execute them, to update the artifact and to disseminate it if necessary, for the continuation of the execution. Moreover, actors potentially have only a partial perception of processes in which they are involved. In practice, this means that certain tasks can be carried out confidentially.

==> declaration-authorship/declaration-authorship.tex <==
%\myChapterStar{Titre}{Titre court}{Ajouter à la table des matières? (false|true|chapter|section|subsection|subsubsection -chapter par défaut-)}
\myChapterStar{Declaration of Authorship}{}{false}

I, the undersigned student \textsc{ZEKENG NDADJI Milliam Maxime}, registration number CM04-10SCI1755, declare that this thesis submitted in fulfilment of the requirements for obtaining the degree of \textit{Doctor/PhD} in Computer Science, option \textit{Software Engineering}, speciality \textit{Business Process Management}, is the result of my own work unless otherwise referenced or acknowledged.

~

\begin{center}
	\textbf{The Student}
	
	~
	
	~
	
	~
	
	\textbf{\textsc{ZEKENG NDADJI Milliam Maxime}}
	
	Date: ...................................
\end{center}

~

\begin{center}
	\textbf{The Co-Directors}
\end{center}

~

~

~

%\begin{multicols}{2}
\hspace{-7mm}
\parbox[c]{.5\textwidth}{
	%\begin{minipage}
		\begin{center}
			\textbf{\textsc{TCHOUP\'E TCHENDJI Maurice}}
			
			\textit{Senior Lecturer, University of Dschang, Cameroon}
			
			Date: ...................................
		\end{center}
	%\end{minipage}
}
	%\columnbreak
\parbox[c]{.5\textwidth}{
	%\begin{minipage}
		\begin{center}
			\textbf{\textsc{TAYOU DJAMEGNI Cl\'ementin}}
			
			\textit{Full Professor, University of Dschang, Cameroon}
			
			Date: ...................................
		\end{center}
	%\end{minipage}
}
%\end{multicols}






==> other-pages/thesis-title.tex <==
\myChapterStar{}{}{false}
\begin{center}
\chaptitlefont %\hrule height 1.5pt
\begin{center}\textcolor{black}{\textsc{Une Approche Grammaticale d'Edition Coop\'erative entre pairs sur une Architecture Orient\'ee Service}}
\end{center}
\end{center}
\vspace{8mm}
\textcolor{black}{\hrule height 4.5pt}%
\vspace{1mm}
\textcolor{black}{\hrule height 1.5pt}


==> resume/resume.tex <==
\let\oldprintchaptertitle=\printchaptertitle
\renewcommand{\printchaptertitle}[1]{%
	\vspace*{-75pt}
	\oldprintchaptertitle{#1}
}%
\myChapterStar{Résumé}{}{section}
\let\printchaptertitle=\oldprintchaptertitle
Dans cette thèse, nous nous intéressons à la conception et à l'implémentation des systèmes workflows distribués, dédiés à l'automatisation des processus opérationnels dits administratifs. Nous proposons une approche de mise en oeuvre de tels systèmes en nous appuyant sur les concepts de systèmes multi-agents, d'architecture Pair à Pair (P2P, égal à égal), d'architecture orientée service et d'édition coopérative de documents structurés (artefacts). 
En effet, nous développons des outils mathématiques permettant à tout concepteur de systèmes workflows, d'exprimer chaque processus administratif qu'il désire automatiser, sous forme d'une grammaire attribuée dont les symboles représentent les tâches à exécuter, les productions spécifient un ordonnancement de celles-ci, et les instances (les arbres de dérivation qui lui sont conformes) représentent les différents scénarii d'exécution menant aux différents états qui matérialisent l'accomplissement des objectifs de l'entreprise. Le modèle grammatical obtenu est ensuite introduit dans un système P2P que nous proposons, et qui est chargé d'assurer l'exécution complètement décentralisée d'instances du processus sous-jacent. 
Ledit système orchestre l'exécution d'une instance de processus sous forme d'une chorégraphie durant laquelle, divers agents logiciels pilotés par des agents humains (acteurs), se coordonnent à l'aide d'artefacts qu'ils éditent collégialement. Les artefacts échangés représentent la mémoire du système: ils donnent des informations sur les tâches déjà exécutées, sur celles prêtes à l'être et sur leurs exécutants. Les agents logiciels sont autonomes et identiques: ils exécutent le même et unique protocole à chaque fois qu'ils reçoivent un artefact. Ce protocole leur permet d'identifier les tâches qu'ils doivent exécuter dans l'immédiat, de les exécuter, de mettre à jour l'artefact et de le diffuser si nécessaire, pour la continuation du processus d'exécution. 
En outre, les acteurs n'ont potentiellement qu'une perception partielle des processus dans lesquels ils sont impliqués. Ce qui autorise donc une possible exécution confidentielle de certaines tâches en pratique: cette propriété permet d'offrir une gestion automatique des processus administratifs se rapprochant un peu plus, de leur gestion non informatisée.

\vspace{1cm}
\noindent\textbf{Mots clés:} Workflows Administratifs, Artefacts, Pair à Pair, Réplique Partielle, Gestion des Processus Opérationnels.

\myCleanStarChapterEnd


